Life span of SAT techniques

In this paper we take 4 different features of the SAT solver CaDiCaL, blocked clause elimination, vivification, on-the-fly self subsumption, and increasing the bound of variable elimination over the SAT Competitions benchmarks between 2009 and 2022. We study these features by both activating them one-by-one and deactivating them one-by-one. We have three hypothesis regarding the experiments: (i) disabling features is always harmful; (ii) the life span of the techniques is limited; and (iii) features simulate each other. Our experiments cannot confirm any of the hypothesis.

==> tables/table1.tex <==
\begin{tabular}{lrrrrrrrrrrr}
\toprule
{} &  2009 &  2011 &  2013 &  2014 &  2015 &  2017 &  2018 &  2019 &  2020 &  2021 &  2022 \\
\midrule
\#Benchmarks    &   292 & 300.0 &   276 & 300.0 &   300 & 350.0 &   400 & 400.0 & 400.0 & 400.0 &   400 \\
default+BCE    &   227 & 234.0 &   233 & 248.0 &   272 & 234.0 &   272 & 231.0 & 220.0 & 259.0 &   261 \\
default        &   229 & 232.0 &   236 & 246.0 &   269 & 235.0 &   271 & 243.0 & 230.0 & 257.0 &   259 \\
default-vivify &   230 & 237.0 &   240 & 249.0 &   272 & 239.0 &   269 & 233.0 & 231.0 & 262.0 &   263 \\
default-OTFS   &   229 & 239.0 &   230 & 242.0 &   269 & 236.0 &   268 & 235.0 & 228.0 & 259.0 &   263 \\
default-BVE+   &   227 & 234.0 &   225 & 245.0 &   268 & 233.0 &   267 & 237.0 & 233.0 & 262.0 &   278 \\
\bottomrule
\end{tabular}


==> tables/table2.tex <==
\begin{tabular}{lrrrrrrrrrrr}
\toprule
{} &  2009 &  2011 &  2013 &  2014 &  2015 &  2017 &  2018 &  2019 &  2020 &  2021 &  2022 \\
\midrule
\#Benchmarks &   292 & 300.0 &   276 & 300.0 &   300 & 350.0 &   400 & 400.0 & 400.0 & 400.0 &   400 \\
base        &   229 & 239.0 &   220 & 236.0 &   262 & 238.0 &   269 & 243.0 & 229.0 & 262.0 &   263 \\
base+vivify &   228 & 236.0 &   222 & 237.0 &   268 & 232.0 &   265 & 241.0 & 231.0 & 261.0 &   262 \\
base+OTFS   &   229 & 237.0 &   221 & 239.0 &   262 &   NaN &   270 & 238.0 & 229.0 & 262.0 &   265 \\
base+BVE+   &   232 & 236.0 &   231 & 242.0 &   266 &   NaN &   266 & 236.0 & 223.0 & 253.0 &   260 \\
base+BCE    &   226 & 237.0 &   221 & 235.0 &   258 & 228.0 &   248 & 237.0 & 230.0 & 261.0 &   259 \\
\bottomrule
\end{tabular}

